Questions Are All You Need to Train a Dense Passage Retriever

We introduce ART, a new corpus-level autoencoding approach for training dense retrieval models that does not require any labeled training data. Dense retrieval is a central challenge for open-domain tasks, such as Open QA, where state-of-the-art methods typically require large supervised datasets with custom hard-negative mining and denoising of positive examples. ART, in contrast, only requires access to unpaired inputs and outputs (e.g. questions and potential answer documents). It uses a new document-retrieval autoencoding scheme, where (1) an input question is used to retrieve a set of evidence documents, and (2) the documents are then used to compute the probability of reconstructing the original question. Training for retrieval based on question reconstruction enables effective unsupervised learning of both document and question encoders, which can be later incorporated into complete Open QA systems without any further finetuning. Extensive experiments demonstrate that ART obtains state-of-the-art results on multiple QA retrieval benchmarks with only generic initialization from a pre-trained language model, removing the need for labeled data and task-specific losses.

==> table/methodology-cmp.tex <==
% !TeX root = ../main.tex
% !TeX spellcheck


\begin{table*}[t]
\small
\centering
\setlength{\tabcolsep}{0.30em}
\begin{tabular}{@{}l | c c c c | c c c c@{}}
 \toprule
 \multicolumn{1}{c}{\textbf{}} & \multicolumn{3}{c}{\textbf{Training Data}} & \multicolumn{4}{c}{\textbf{Training Methodology}} \\
 \midrule
 \multirow{2}{2.5cm}{\textbf{Model}} & \multirow{2}{1.3cm}{\textit{Unlabeled Text}} & \multirow{2}{1.3cm}{\textit{Question-Passages}} & \multirow{2}{1.3cm}{\textit{Questions}} & \multirow{2}{1.3cm}{\textit{Question-Answers}} & \multirow{2}{1.3cm}{\textit{Hard Negatives}} & \multirow{2}{1.4cm}{\textit{In-Batch Negatives}} & \multirow{2}{1.3cm}{\textit{PLM Feedback}} & \multirow{2}{1.4cm}{\textit{PLM Finetuning}} \\
 & & & & & & & \\
 \midrule
 ICT~\citep{lee-etal-2019-latent}   & \cmark &   &  &  &  & \cmark &  &  \\
 REALM~\citep{guu2020realm} & \cmark &   &  &  &  &  & \cmark & \cmark \\
 Spider~\cite{ram2021learning} & \cmark & & & &  & \cmark & & \\
 DPR~\citep{karpukhin2020dense}     &  & \cmark &   & & \cmark & \cmark & &  \\
 ANCE~\cite{xiong2021approximate}   & & \cmark & &  & \cmark & \cmark & & \\
 RocketQA~\cite{qu-etal-2021-rocketqa} & \cmark & \cmark & \cmark & & \cmark & \cmark & \cmark & \cmark \\
 EMDR$^2$~\cite{sachan2021endtoend} & & &   & \cmark & & & \cmark & \cmark \\
 \midrule
 \model{} (Our Approach) & \cmark & & \cmark & &  &  & \cmark & \\
 \bottomrule
\end{tabular}
\caption{A comparison of recent dense retriever training approaches.
These approaches are grouped under two buckets: the kind of data used and the methodology adopted during training.
\textbf{PLM} stands for pre-trained language model.
\textbf{Unlabeled Text} indicates whether unlabeled text data such as Wikipedia was used during training. 
\textbf{Question-Passages} indicates if training requires collection of questions and aligned passages. 
\textbf{Questions} indicates whether a collection of questions were used during training. 
\textbf{Hard Negatives} denotes if additionally mined hard negative examples were used in training.
\textbf{In-Batch Negatives} indicates whether the positive passages of other questions were used as negative examples. 
\textbf{PLM Feedback} denotes whether the retriever gets relevance feedback from the PLM to update its parameters.
\textbf{PLM Finetuning} indicates if the PLM is finetuned or not.
}
\label{tab:summary-comparison}
\end{table*}

